TADACap: Time-series Adaptive Domain-Aware Captioning

While image captioning has gained significant attention, the potential of captioning time-series images, prevalent in areas like finance and healthcare, remains largely untapped. Existing time-series captioning methods typically offer generic, domain-agnostic descriptions of time-series shapes and struggle to adapt to new domains without substantial retraining. To address these limitations, we introduce TADACap, a retrieval-based framework to generate domain-aware captions for time-series images, capable of adapting to new domains without retraining. Building on TADACap, we propose a novel retrieval strategy that retrieves diverse image-caption pairs from a target domain database, namely TADACap-diverse. We benchmarked TADACap-diverse against state-of-the-art methods and ablation variants. TADACap-diverse demonstrates comparable semantic accuracy while requiring significantly less annotation effort.

==> sec6_discussion.tex <==
\section{Discussion}
In comparison to retrieving diverse samples from the target domain database, SmallCap~\cite{ramos2022smallcap} retrieves similar samples to the query image. The underlying assumption of the retrieval step is that CLIP image embedding of the query image is similar to the CLIP text embeddings of captions of similar images, which means that the deployed CLIP model should have learned the visual concepts in the query image and the language concepts in the datastore captions during pre-training. For example, in one of the SmallCap experiments, CLIP was able to associate the image embedding of pink dress to "tutu" caption in Flickr30k dataset, thus SmallCap can adapt the output caption to use "tutu" to describe the pink dress when using Flickr30k as the retrieval database. This underlying assumption of CLIP is valid for visual and language concepts in natural images, i.e., the type of images that CLIP was pre-trained on (\doblue{is this true?}). However, this assumption does not necessarily hold for the time-series domain, because CLIP was not pre-trained on such data, and no large time-series image-caption dataset exists yet for sufficient pretraining. In our work, we don't rely on such assumption and showed the effectiveness of using diverse samples from target domain database.

